Syntax and semantics of focalisation with relative monads and comonads

The logical principles of focalisation and polarisation can be used to design well-behaved term syntaxes for sequent calculus, which play a role as meta-languages for describing effectful computation. On the semantics side, this corresponds to an axiomatic and polarised notion of model of computation stated in terms of adjunctions over non-associative categories. In this paper, we study the special and delicate cases of resource and effect modalities in a general intuitionistic and linear setting: an exponential comonad $!$ (refining $\square$) and a strong monad $\lozenge$. The starting point of our contribution is noticing that the completeness for a polarised syntax for $!$ and $\lozenge$ with respect to (co)monads in linear call-by-push-value models can be achieved if we move to relative (co)monads: more precisely, comonads relative to $\downarrow$ (the positive shift functor) for $!$ and monads relative to $\uparrow$ (the negative shift functor) for $\lozenge$. These specialisations of the concept of relative (co)monad to call-by-push-value adjunctions recently appeared. Yet the syntax we present arose from proof-theoretic consideration, without the link with relative (co)monads being noticed at the time. Our first remark is thus that (co)monads relative to a call-by-push-value adjunction have been motivated previously from a proof-theoretic perspective in the context of focalisation, which also provides a meta-language for these concepts in an effectful setting. We carry out the study of these modalities from the axiomatic, non-associative point of view. We recall the notion of adjunction over non-associative categories, and establish correspondence results between this notion of adjunction and that of relative adjunction. This correspondence is then extended to linear-non-linear and strong versions of adjunctions as needed to model $!$ and $\lozenge$.

==> includes/macros5unstable.tex <==
\selectlanguage{english}\input{includes/lyxproofs.tex}\input{includes/lyxymatrix.tex}\global\long\def\Operatorname#1{\operatorname{#1}}

\global\long\def\rotxc#1{\begin{sideways}#1\end{sideways}}

\global\long\def\invert#1{\hbox{\rotxc{\rotxc{\ensuremath{#1}}}}}

\global\long\def\lyxmathchoice#1#2#3#4{\mathchoice{#1}{#2}{#3}{#4}}

\global\long\def\mathraise#1#2#3#4{\lyxmathchoice{\raisebox{#2}{${\displaystyle {#1}}$}}{\raisebox{#2}{$#1$}}{\raisebox{#3}{${\scriptstyle {#1}}$}}{\raisebox{#4}{${\scriptscriptstyle {#1}}$}}}

\global\long\def\mathraiseord#1#2#3#4{\mathord{\mathraise{#1}{#2}{#3}{#4}}}

\global\long\def\ltxifnextchar{\csname@ifnextchar\endcsname}

\global\long\def\df{\iffontspec\eqdef\else\overset{\raisebox{-0.4ex}{\ensuremath{{\scriptscriptstyle \textup{def}}}}}{=}\fi}

\global\long\def\set#1#2{\perfectbinary{IncreaseHeight}\{|\}{#1\mathrel{}}{\mathrel{}#2}}

\global\long\def\shpos{\mathraiseord{\downarrow}{0.22ex}{0.14ex}{0.11ex}\ltxifnextchar\shneg{\mkern-2.8mu  }{}}

\global\long\def\shneg{\mathraiseord{\uparrow}{0.29ex}{0.21ex}{0.14ex}\ltxifnextchar\shpos{\mkern-2.8mu  }{}}

\global\long\def\Shpos{\mathraiseord{\Downarrow}{0.2ex}{0.15ex}{0.09ex}\ltxifnextchar\Shneg{\iffontspec\mkern-5.3mu  \else\mkern-2.5mu  \fi}{}}

\global\long\def\Shneg{\mathraiseord{\Uparrow}{0.28ex}{0.21ex}{0.14ex}\ltxifnextchar\Shpos{\iffontspec\mkern-5mu  \else\mkern-2.5mu  \fi}{}}

\global\long\def\wpar{\mathbin{\iffontspec\upand\else\invert{\&}\fi}}

\global\long\def\oc{\mathord{!}}

\global\long\def\ocv{\mathord{\textrm{\textup{!`}}}}

\global\long\def\wn{\mathord{?}}

\global\long\def\with{\mathbin{\&}}

\global\long\def\falso{\mathbf{\boldsymbol{0}}}

\global\long\def\unite{\mathbf{\boldsymbol{1}}}

\global\long\def\mixarrow{\rightarrowtriangle}

\global\long\def\system#1{\mathbf{#1}}

\global\long\def\LL{\system{LL}}

\global\long\def\ILL{\system{ILL}}

\global\long\def\LK{\system{LK}}

\global\long\def\LLP{\system{LLP}}

\global\long\def\LC{\system{LC}}

\global\long\def\LJ{\system{LJ}}

\global\long\def\NJ{\system{NJ}}

\global\long\def\MALL{\system{MALL}}

\global\long\def\LU{\system{LU}}

\global\long\def\polsystem#1{\texorpdfstring{{\system{#1}^{\mathrlap{\eta}}}_{\mkern-1.5mu  p}}{#1\eta p}}

\global\long\def\MLJp{\polsystem{MLJ}}

\global\long\def\IMLLp{\polsystem{IMLL}}

\global\long\def\LJp{\polsystem{LJ}}

\global\long\def\IMALLp{\polsystem{IMALL}}

\global\long\def\IMELLp{\polsystem{IMELL}}

\global\long\def\ILLp{\polsystem{ILL}}

\global\long\def\LKp{\polsystem{LK}}

\global\long\def\LLp{\polsystem{LL}}

\global\long\def\subtype{\mathrel{\mathord{<}\mkern-1.5mu  {\vcentcolon}}}

\global\long\def\otimescriptstyle{{\raisebox{0.07ex}{\hbox{\mbox{\ensuremath{{\scriptstyle \otimes}}}}}}}

\global\long\def\otimescriptscriptstyle{{\raisebox{0.05ex}{\hbox{\mbox{\ensuremath{{\scriptscriptstyle \otimes}}}}}}}

\global\long\def\smallotimes{\mkern1mu  {\lyxmathchoice{\otimescriptstyle}{\otimescriptstyle}{\otimescriptscriptstyle}{\otimescriptscriptstyle}}\mkern1mu  }

\global\long\def\keyword#1{\Operatorname{\textsf{#1}}}

\global\long\def\bnf{\iffontspec\Coloneq\else\Coloneqq\fi}

\global\long\def\bmid{\mathrel{\boldsymbol{\nthleft{1}|}}}

\global\long\def\moins{\circleddash}

\global\long\def\plus{+}

\global\long\def\push{\mathord{\cdot}}

\global\long\def\pleft{\pi_{1}}

\global\long\def\pright{\pi_{2}}

\global\long\def\pith{\pi_{i}}

\global\long\def\ppair#1#2{{<}\mspace{1mu}#1\mspace{1mu}\mathord{;}\mspace{3mu}#2\mspace{1mu}{>}}

\global\long\def\ileft{\iota_{1}}

\global\long\def\iright{\iota_{2}}

\global\long\def\iith{\iota_{i}}

\global\long\def\mt{\smash{\tilde{\mu}}\vphantom{\mu}}

\global\long\def\lmmt{\bar{\lambda}\mu\mt}

\global\long\def\mustar{\mu\mathord{\star}}

\global\long\def\cut#1#2{\cutprimitive{#1}{#2}}

\global\long\def\Bra#1{\cutbraprimitive{#1}}

\global\long\def\Ket#1{\cutketprimitive{#1}}

\global\long\def\parens#1{\perfectparens{#1}}

\global\long\def\tphat{{\raisebox{-0.5ex}{\hbox{\ensuremath{\hat{\hphantom{e}}}}}}}

\global\long\def\muhat{\hat{\mu}}

\global\long\def\contor#1#2#3#4{\perfectcase{{#1.}#2\mkern2mu  }{\mkern2mu  {#3.}#4}}

\global\long\def\mui#1#2#3#4{\mt\contor{#1}{#2}{#3}{#4}}

\global\long\def\mupair#1#2#3#4{\mu\ppair{{#1}.#2}{{#3}.#4}}

\global\long\def\term#1{\mu{{<}#1{>}}}

\global\long\def\init#1{\mt[#1]}

\global\long\def\curlybraces#1{\perfectunary{CurrentHeight}\lbrace\rbrace{#1}}

\global\long\def\brackets#1{\perfectbrackets{#1}}

\global\long\def\substslash#1#2{\csname cut@computeBinary@CurrentHeightPlusOne\endcsname{}{#1}{\nthmiddle{\csname cut@n\endcsname}/}{#2}{}}

\global\long\def\bracketsmid#1#2{\csname cut@computeBinary@CurrentHeightPlusOne\endcsname{}{#1}{\mathbin{\nthmiddle{\csname cut@n\endcsname}|}}{#2}{}}

\global\long\def\subst#1#2{\perfectunary{CurrentHeightPlusOne}[]{\substslash{#1}{#2}}}

\global\long\def\expsubst#1#2{\perfectunary{CurrentHeightPlusOne}\{\}{\substslash{#1}{#2}}}

\global\long\def\mkernsp#1#2{\ltxifnextchar#2{\csname mkern\endcsname#1}{}}

\global\long\def\varp#1{#1^{{\mkern-1mu  \mathord{\plus}\mkern-2mu  }}\mkernsp{-3mu}.}

\global\long\def\varn#1{#1^{{\moins}\mkern-1mu  }\mkernsp{-3mu}.}

\global\long\def\termp#1{#1_{\smash{\plus}}}

\global\long\def\termn#1{#1_{\smash{\moins}}}

\global\long\def\eps#1{\varepsilon_{#1}}\global\long\def\epsprime#1{\varepsilon'_{#1}}

\global\long\def\vareps#1#2{#1^{\mkern0.5mu  {\eps{#2}}\mkern-1mu  }\mkernsp{-2mu}.}

\global\long\def\termeps#1#2{#1_{\smash{\eps{#2}}}}

\global\long\def\varepsprime#1#2{#1^{\mkern0.5mu  {\epsprime{#2}}\mkern-1mu  }\mkernsp{-2mu}.}

\global\long\def\termepsprime#1#2{#1_{\smash{\epsprime{#2}}}}

\global\long\def\tbrack#1{\curlybraces{#1}}

\global\long\def\ebrack#1{\curlybraces{#1}}

\global\long\def\mtbrack#1{\mt\{#1\}}

\global\long\def\mubrack#1{\mu\{#1\}}

\global\long\def\letin#1{\keyword{let}#1\keyword{in}}

\global\long\def\matchwith#1{\keyword{match}#1\keyword{with}}

\global\long\def\be{\keyword{be}}

\global\long\def\addsubst#1#2{,\substslash{#1}{#2}}

\global\long\def\variableset#1#2{\Operatorname{\textbf{#1}}{#2}}

\global\long\def\v#1{\variableset v{#1}}

\global\long\def\fv#1{\variableset{fv}{#1}}

\global\long\def\Bracks#1{[\mkern-3mu  [#1]\mkern-3mu  ]}

\global\long\def\dispatch#1#2#3#4#5{\delta(#1,\allowbreak#2.#3,\allowbreak#4.#5)}

\global\long\def\L{\system L}

\global\long\def\argrel#1#2#3{\mathrel{#3_{\cramped{\textup{#1}\ifx\empty#1\empty#2\else_{#2}\fi}}}}

\global\long\def\argred#1#2{\argrel{#1}{#2}{\vartriangleright}}

\global\long\def\argnred#1#2{\iffontspec\argrel{#1}{#2}{\nvartriangleright}\else\argrel{#1}{#2}{\not\vartriangleright}\fi}

\global\long\def\argredinv#1#2{\argrel{#1}{#2}{\vartriangleleft}}

\global\long\def\argRed#1#2{\argrel{#1}{#2}{\rightarrow}}

\global\long\def\argRedinv#1#2{\argrel{#1}{#2}{\leftarrow}}

\global\long\def\argPar#1#2{\argrel{#1}{#2}{\Rightarrow}}

\global\long\def\argParinv#1#2{\argrel{#1}{#2}{\Leftarrow}}

\global\long\def\argreds#1#2{\argrel{#1}{#2}{\vartriangleright^{\ast}}}

\global\long\def\argredinvs#1#2{\argrel{#1}{#2}{\vartriangleleft^{\ast}}}

\global\long\def\argReds#1#2{\argrel{#1}{#2}{\rightarrow^{\ast}}}

\global\long\def\argRedinvs#1#2{\argrel{#1}{#2}{\leftarrow^{\ast}}}

\global\long\def\argPars#1#2{\argrel{#1}{#2}{\Rightarrow^{\ast}}}

\global\long\def\argParinvs#1#2{\argrel{#1}{#2}{\Leftarrow^{\ast}}}

\global\long\def\argeq#1#2{\argrel{#1}{#2}{\simeq}}

\global\long\def\argneq#1#2{\iffontspec\argrel{#1}{#2}{\nsimeq}\else\argrel{#1}{#2}{\not\simeq}\fi}

\global\long\def\machred#1{\succ_{#1}}

\global\long\def\machredinv#1{\prec_{#1}}

 
\global\long\def\group#1{{#1}}

\global\long\def\visiblelefteqn#1{\lefteqn{#1}}

\global\long\def\mathcomment#1{\{\}}

\global\long\def\proofsep{\mathrel{\vphantom{(\mid c'}{\vdash}}}

\global\long\def\cond#1{\tag{\ensuremath{#1}}}

\global\long\def\relrel#1{\mathord{}\mathrel{#1}\mathord{}}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

\global\long\def\abs#1{\left|#1\right|}

\global\long\def\norm#1{\left\Vert #1\right\Vert }

\global\long\def\dom#1{\Operatorname{dom}#1}

\global\long\def\id{\mathrm{id}}

\global\long\def\Id{\mathrm{Id}}

\global\long\def\idfunctor{1}

\global\long\def\obj#1{\abs{#1}}

\global\long\def\op#1{{#1}^{\textup{op}}}

\global\long\def\inv#1{#1^{-1}}

\global\long\def\restr#1#2{{#1_{\upharpoonright#2}}}

\global\long\def\dfequiv{\overset{{\scriptscriptstyle \textrm{def}}}{\Longleftrightarrow}}

\global\long\def\reflect{\mathbin{\triangleleft}}

\global\long\def\sha#1{#1^{\sharp}}

\global\long\def\fla#1{#1^{\flat}}

\global\long\def\adj#1{#1^{\ast}}

\global\long\def\Set#1{\big\{#1\big\}}

\global\long\def\setmid{\,\big|\,}

\global\long\def\C{\mathscr{C}}

\global\long\def\Ccal{\mathcal{C}}

\global\long\def\scL{\mathscr{L}}

\global\long\def\scC{\mathscr{C}}

\global\long\def\scV{\mathscr{V}}

\global\long\def\bbN{\iffontspec\BbbN\else\mathbb{N}\fi}

\global\long\def\to{\mathbin{\rightarrow}}

\global\long\def\dotarrow{\mathrel{\mkern-2mu  \dot{\mkern2mu  \rightarrow}}}

\global\long\def\nattransf{\dotarrow}

\global\long\def\ddotarrow{\mathrel{\!\ddot{\,\rightarrow}}}

\global\long\def\embed{\hookrightarrow}

\global\long\def\simrightarrow{\iffontspec\similarrightarrow\else\stackrel{\sim}{\rightarrow}\fi}

\global\long\def\farrow#1#2#3{#2\xrightarrow{#1}#3}

\global\long\def\farr#1{\mathrel{{\relbar}\raisebox{0.2ex}{\ensuremath{{\scriptstyle #1}}}\mkern-1mu  {\rightarrow}}}

\global\long\def\stackrightleftarrows#1#2{\mathrel{\underset{#2}{\overset{#1}{\rightleftarrows}}}}

\global\long\def\stackleftrightarrows#1#2{\mathrel{\underset{#2}{\overset{#1}{\leftrightarrows}}}}

\global\long\def\labelrightarrowcompact#1{\mathrel{\xrightarrow{#1}}}

\def\labelrightarrowcompact#1#2{\mbox{$#1\ifx#1\textstyle \clipbox{0em 0em {.4\width} 0em}{$\vphantom{A}{\relbar}$}\mkern0mu\raisebox{0.3ex}{$\scriptstyle#2$}\mkern0mu\clipbox{{.3\width} 0em 0em 0em}{$\rightarrow$}\else \xrightarrow{#2}\fi $}}

\global\long\def\labelrightarrow#1{\mathbin{\mathpalette\labelrightarrowcompact{#1}}}

\global\long\def\morphism#1{\labelrightarrow{#1}}

\global\long\def\natiso{\mathrel{{\textstyle \cong}}}

\global\long\def\spancols#1#2{\csname multicolumn\endcsname{#2}{c}{#1}}

\global\long\def\spanrows#1#2{\multirow{#2}{*}{\ensuremath{#1}}}

\global\long\def\spancolsleft#1#2{\csname multicolumn\endcsname{#2}{l}{#1}}

\global\long\def\spantwo#1{\csname multicolumn\endcsname{2}{c}{#1}}

\global\long\def\linespacing#1{\rule[-#1]{0pt}{0pt}}

\global\long\def\mathvspace{\vphantom{\rule{0pt}{1.75em}}}

\global\long\def\qedmultiline{\tag*{\qedhere}}

\global\long\def\where{\;\quad\text{where}\;\quad}

\global\long\def\when{\;\quad\text{when}\;\quad}

\global\long\def\textor{\;\quad\text{or}\;\quad}

\global\long\def\addstretchamount{2.5}

\global\long\def\addsmallstretchamount{1.3}

\newcommandx\addcustomstretch[3][usedefault, addprefix=\global, 1=\addstretchamount, 2=0.0em]{\begingroup\edef\arraystretch{#1}\addtolength\arraycolsep{#2}#3\endgroup}

\global\long\def\addstretch#1{\addcustomstretch[\addstretchamount][0.0em]{#1}}

\global\long\def\addsmallstretch#1{\addcustomstretch[\addsmallstretchamount][-0.4em]{#1}}

\global\long\def\removestretch#1{\addcustomstretch[1.0][-4pt]{#1}}

\global\long\def\prom#1{\oc{#1}}

\global\long\def\vdashsubscript#1{\mathrel{{\vdash}\!{\ensuremath{_{#1}}}}}

\global\long\def\focvdash{\mathrel{\vdashsubscript f}}

\global\long\def\diam#1{\group{#1}^{\diamond}}

\global\long\def\colon{\mskip1muplus4muminus2mu\mathord{:}\mskip1muplus4muminus2mu}

\global\long\def\ech#1{\perfectbrackets{#1}}

\global\long\def\fresh{\mathrel{\#}}

\global\long\def\varpm#1{#1^{{\pm}}\mkernsp{-3mu}.}

\global\long\def\cs#1#2{#1^{#2\mkern-1mu  }\mkernsp{-3.5mu}.}

\global\long\def\push{\mathord{\cdot}}

\global\long\def\Li{\system L_{\text{int}}}

\global\long\def\yon{\mathbf{y}}

\global\long\def\pcomp{\mathbin{\iffontspec\vysmblkcircle\else\bullet\fi}}

\global\long\def\ncomp{\mathbin{\iffontspec\vysmwhtcircle\else\circ\fi}}

\global\long\def\pair#1#2{\langle#1,#2\rangle}

\global\long\def\dotcirc{\ifx\fisheye\undefined\mathbin{\visiblelefteqn{\mspace{2.4mu}\mathord{\cdotp}}\mathord{\ncomp}}\else\mathbin{\fisheye}\fi}

\global\long\def\polarity{\varpi}

\global\long\def\swash#1{\iffontspec{\text{\fontspec[Style=Swash,Scale=MatchLowercase]{Arno Pro Bold Italic}#1}}\else\boldsymbol{\textrm{\textbf{\textit{#1}}}}\fi}

\def\swasharg#1{\ensuremath{\mathbcal{#1}\mkern-0.5mu}}\def\swash#1{\textbf{\textit{\swasharg #1}}}

\global\long\def\catstyle#1{\swash{#1}}

\global\long\def\Setcat{\catstyle{Set}}

\global\long\def\Cat{\catstyle{Cat}}

\global\long\def\Dupl{\catstyle{Dupl}}

\global\long\def\Adj{\catstyle{Adj}}

\global\long\def\Tf{\catstyle{Tf}}

\global\long\def\profunctor#1#2{\op{#1}\times#2\rightarrow\Setcat}

\global\long\def\extlambda#1#2{\widehat{#2}.#1}

\global\long\def\D{\mathscr{D}}

\global\long\def\N{\mathscr{N}}

\global\long\def\P{\mathscr{P}}

\global\long\def\psh#1{\widehat{#1}}

\global\long\def\enr#1{\underline{#1\mspace{-1mu}}\mspace{1mu}}

\global\long\def\orth#1{{{#1}^{\bot}}}

\global\long\def\biorth#1{{{#1}^{\bot\bot}}}

\global\long\def\interp#1{\big|#1\big|}

\global\long\def\interpv#1{\big\|#1\big\|}

\providecommand{\Vbar}{\mathord{\bot\mkern-10.5mu\bot}}

\global\long\def\Vbar{\mathord{\bot\mkern-10.5mu  \bot}}

\global\long\def\Bot{\mathord{\Vbar}}

\global\long\def\polar{\mathrel{\Bot}}

\global\long\def\nBot{\mathrel{\not\mkern-1.6mu  \polar}}

\global\long\def\padifnempty#1{\ifx\empty#1\empty\else\mkern2mu  #1^{\mkern0.5mu  }\mkern2mu  \fi}

\global\long\def\xyadjnoresize#1#2#3#4#5{\Xymatrixone\xymatrix{#1\ \ar@<0.8ex>[r]|-(.275){#2}\ar@{}@<0.1ex>[r]|-{\scriptscriptstyle #5}  &  \ar@<0.6ex>[l]|-(.275){#3}\ #4}
 }

\global\long\def\xyadjinline#1#2#3#4{\xyresize[][\ifx\empty#2#3\empty1pc\else25pt\fi]{\xyadjnoresize{#1}{\padifnempty{#2}}{\padifnempty{#3}}{#4}{\bot}}}

\global\long\def\xyadjdisplay#1#2#3#4{\xymatrix{#1\ \ar@<1ex>[r]\sp-{#2}\ar@{}[r]|-\bot &  \ar@<1ex>[l]\sp-{#3}\ #4}
 }

\global\long\def\xyadj#1#2#3#4{\mathchoice{\xyadjdisplay{#1}{#2}{#3}{#4}}{\xyadjinline{#1}{#2}{#3}{#4}}{\xyadjinline{#1}{#2}{#3}{#4}}{\xyadjinline{#1}{#2}{#3}{#4}}}

\makeatletter
\def\underline@size#1#2{\setbox0=\hbox{$\m@th#1#2$}\rlap{\resizebox*{\wd0}{\totalheight}{\raisebox{-\dp0}{\hbox{\normalfont\_}}}}\box0}
\def\underline{\mathpalette\underline@size}
\makeatother
\global\def\dashedScoreFiller{\hbox{\raisebox{-0.4ex}[0.1em][0pt]{\normalfont\hspace{0.1em}\textendash\hspace{0.1em}}}}
\global\def\ruleScoreFiller{\hbox{}\hskip0pt\raisebox{-0.45ex}[0.1ex][0pt]{\resizebox{\displace}{\height}{\hbox{\normalfont\textemdash}}}
}
\newcommand{\hlinesmooth}[1]{\raisebox{-0.45ex}[0.1ex][0pt]{\resizebox{#1}{\height}{\hbox{\normalfont\textemdash}}}}
\newcommand{\hlinemed}{\vskip\baselineskip \noindent \hspace*{\fill}\hlinesmooth{0.62\linewidth}
  \hspace*{\fill}}
\newcommand{\hlinefill}{\vskip0.5\baselineskip \noindent \hspace*{\fill}\hlinesmooth{\linewidth}
  \hspace*{\fill}\vskip-1.4\baselineskip }\selectlanguage{british}



==> includes/systemlyx.tex <==
\global\long\def\Operatorname#1{\operatorname{#1}}

\global\long\def\rotxc#1{\begin{sideways}#1\end{sideways}}

\global\long\def\invert#1{\hbox{\rotxc{\rotxc{\ensuremath{#1}}}}}

\global\long\def\lyxmathchoice#1#2#3#4{\mathchoice{#1}{#2}{#3}{#4}}

\global\long\def\mathraise#1#2#3#4{\lyxmathchoice{\raisebox{#2}{${\displaystyle {#1}}$}}{\raisebox{#2}{$#1$}}{\raisebox{#3}{${\scriptstyle {#1}}$}}{\raisebox{#4}{${\scriptscriptstyle {#1}}$}}}

\global\long\def\mathraiseord#1#2#3#4{\mathord{\mathraise{#1}{#2}{#3}{#4}}}

\global\long\def\ltxifnextchar{\csname@ifnextchar\endcsname}

\global\long\def\df{\iffontspec\eqdef\else\overset{\raisebox{-0.4ex}{\ensuremath{{\scriptscriptstyle \textup{def}}}}}{=}\fi}

\global\long\def\set#1#2{\perfectbinary{IncreaseHeight}\{|\}{#1\mathrel{}}{\mathrel{}#2}}

\global\long\def\shpos{\mathraiseord{\downarrow}{0.22ex}{0.14ex}{0.11ex}\ltxifnextchar\shneg{\mkern-2.8mu  }{}}

\global\long\def\shneg{\mathraiseord{\uparrow}{0.29ex}{0.21ex}{0.14ex}\ltxifnextchar\shpos{\mkern-2.8mu  }{}}

\global\long\def\Shpos{\mathraiseord{\Downarrow}{0.2ex}{0.15ex}{0.09ex}\ltxifnextchar\Shneg{\iffontspec\mkern-5.3mu  \else\mkern-2.5mu  \fi}{}}

\global\long\def\Shneg{\mathraiseord{\Uparrow}{0.28ex}{0.21ex}{0.14ex}\ltxifnextchar\Shpos{\iffontspec\mkern-5mu  \else\mkern-2.5mu  \fi}{}}

\global\long\def\wpar{\mathbin{\iffontspec\upand\else\invert{\&}\fi}}

\global\long\def\oc{\mathord{!}}

\global\long\def\ocv{\mathord{\textrm{\textup{!`}}}}

\global\long\def\wn{\mathord{?}}

\global\long\def\with{\mathbin{\&}}

\global\long\def\falso{\mathbf{\boldsymbol{0}}}

\global\long\def\unite{\mathbf{\boldsymbol{1}}}

\global\long\def\mixarrow{\rightarrowtriangle}

\global\long\def\system#1{\mathbf{#1}}

\global\long\def\LL{\system{LL}}

\global\long\def\ILL{\system{ILL}}

\global\long\def\LK{\system{LK}}

\global\long\def\LLP{\system{LLP}}

\global\long\def\LC{\system{LC}}

\global\long\def\LJ{\system{LJ}}

\global\long\def\NJ{\system{NJ}}

\global\long\def\MALL{\system{MALL}}

\global\long\def\LU{\system{LU}}

\global\long\def\polsystem#1{\texorpdfstring{{\system{#1}^{\mathrlap{\eta}}}_{\mkern-1.5mu  p}}{#1\eta p}}

\global\long\def\MLJp{\polsystem{MLJ}}

\global\long\def\IMLLp{\polsystem{IMLL}}

\global\long\def\LJp{\polsystem{LJ}}

\global\long\def\IMALLp{\polsystem{IMALL}}

\global\long\def\IMELLp{\polsystem{IMELL}}

\global\long\def\ILLp{\polsystem{ILL}}

\global\long\def\LKp{\polsystem{LK}}

\global\long\def\LLp{\polsystem{LL}}

\global\long\def\subtype{\mathrel{\mathord{<}\mkern-1.5mu  {\vcentcolon}}}

\global\long\def\otimescriptstyle{{\raisebox{0.07ex}{\hbox{\mbox{\ensuremath{{\scriptstyle \otimes}}}}}}}

\global\long\def\otimescriptscriptstyle{{\raisebox{0.05ex}{\hbox{\mbox{\ensuremath{{\scriptscriptstyle \otimes}}}}}}}

\global\long\def\smallotimes{\mkern1mu  {\lyxmathchoice{\otimescriptstyle}{\otimescriptstyle}{\otimescriptscriptstyle}{\otimescriptscriptstyle}}\mkern1mu  }

\global\long\def\keyword#1{\Operatorname{\textsf{#1}}}

\global\long\def\bnf{\iffontspec\Coloneq\else\Coloneqq\fi}

\global\long\def\bmid{\mathrel{\boldsymbol{\nthleft{1}|}}}

\global\long\def\moins{\circleddash}

\global\long\def\plus{+}

\global\long\def\push{\mathord{\cdot}}

\global\long\def\pleft{\pi_{1}}

\global\long\def\pright{\pi_{2}}

\global\long\def\pith{\pi_{i}}

\global\long\def\ppair#1#2{{<}\mspace{1mu}#1\mspace{1mu}\mathord{;}\mspace{3mu}#2\mspace{1mu}{>}}

\global\long\def\ileft{\iota_{1}}

\global\long\def\iright{\iota_{2}}

\global\long\def\iith{\iota_{i}}

\global\long\def\mt{\smash{\tilde{\mu}}\vphantom{\mu}}

\global\long\def\lmmt{\bar{\lambda}\mu\mt}

\global\long\def\mustar{\mu\mathord{\star}}

\global\long\def\cut#1#2{\cutprimitive{#1}{#2}}

\global\long\def\Bra#1{\cutbraprimitive{#1}}

\global\long\def\Ket#1{\cutketprimitive{#1}}

\global\long\def\parens#1{\perfectparens{#1}}

\global\long\def\tphat{{\raisebox{-0.5ex}{\hbox{\ensuremath{\hat{\hphantom{e}}}}}}}

\global\long\def\muhat{\hat{\mu}}

\global\long\def\contor#1#2#3#4{\perfectcase{{#1.}#2\mkern2mu  }{\mkern2mu  {#3.}#4}}

\global\long\def\mui#1#2#3#4{\mt\contor{#1}{#2}{#3}{#4}}

\global\long\def\mupair#1#2#3#4{\mu\ppair{{#1}.#2}{{#3}.#4}}

\global\long\def\term#1{\mu{{<}#1{>}}}

\global\long\def\init#1{\mt[#1]}

\global\long\def\curlybraces#1{\perfectunary{CurrentHeight}\lbrace\rbrace{#1}}

\global\long\def\brackets#1{\perfectbrackets{#1}}

\global\long\def\substslash#1#2{\csname cut@computeBinary@CurrentHeightPlusOne\endcsname{}{#1}{\nthmiddle{\csname cut@n\endcsname}/}{#2}{}}

\global\long\def\bracketsmid#1#2{\csname cut@computeBinary@CurrentHeightPlusOne\endcsname{}{#1}{\mathbin{\nthmiddle{\csname cut@n\endcsname}|}}{#2}{}}

\global\long\def\subst#1#2{\perfectunary{CurrentHeightPlusOne}[]{\substslash{#1}{#2}}}

\global\long\def\expsubst#1#2{\perfectunary{CurrentHeightPlusOne}\{\}{\substslash{#1}{#2}}}

\global\long\def\mkernsp#1#2{\ltxifnextchar#2{\csname mkern\endcsname#1}{}}

\global\long\def\varp#1{#1^{{\mkern-1mu  \mathord{\plus}\mkern-2mu  }}\mkernsp{-3mu}.}

\global\long\def\varn#1{#1^{{\moins}\mkern-1mu  }\mkernsp{-3mu}.}

\global\long\def\termp#1{#1_{\smash{\plus}}}

\global\long\def\termn#1{#1_{\smash{\moins}}}

\global\long\def\eps#1{\varepsilon_{#1}}\global\long\def\epsprime#1{\varepsilon'_{#1}}

\global\long\def\vareps#1#2{#1^{\mkern0.5mu  {\eps{#2}}\mkern-1mu  }\mkernsp{-2mu}.}

\global\long\def\termeps#1#2{#1_{\smash{\eps{#2}}}}

\global\long\def\varepsprime#1#2{#1^{\mkern0.5mu  {\epsprime{#2}}\mkern-1mu  }\mkernsp{-2mu}.}

\global\long\def\termepsprime#1#2{#1_{\smash{\epsprime{#2}}}}

\global\long\def\tbrack#1{\curlybraces{#1}}

\global\long\def\ebrack#1{\curlybraces{#1}}

\global\long\def\mtbrack#1{\mt\{#1\}}

\global\long\def\mubrack#1{\mu\{#1\}}

\global\long\def\letin#1{\keyword{let}#1\keyword{in}}

\global\long\def\matchwith#1{\keyword{match}#1\keyword{with}}

\global\long\def\be{\keyword{be}}

\global\long\def\addsubst#1#2{,\substslash{#1}{#2}}

\global\long\def\variableset#1#2{\Operatorname{\textbf{#1}}{#2}}

\global\long\def\v#1{\variableset v{#1}}

\global\long\def\fv#1{\variableset{fv}{#1}}

\global\long\def\Bracks#1{[\mkern-3mu  [#1]\mkern-3mu  ]}

\global\long\def\dispatch#1#2#3#4#5{\delta(#1,\allowbreak#2.#3,\allowbreak#4.#5)}

\global\long\def\L{\system L}

\global\long\def\argrel#1#2#3{\mathrel{#3_{\cramped{\textup{#1}\ifx\empty#1\empty#2\else_{#2}\fi}}}}

\global\long\def\argred#1#2{\argrel{#1}{#2}{\vartriangleright}}

\global\long\def\argnred#1#2{\iffontspec\argrel{#1}{#2}{\nvartriangleright}\else\argrel{#1}{#2}{\not\vartriangleright}\fi}

\global\long\def\argredinv#1#2{\argrel{#1}{#2}{\vartriangleleft}}

\global\long\def\argRed#1#2{\argrel{#1}{#2}{\rightarrow}}

\global\long\def\argRedinv#1#2{\argrel{#1}{#2}{\leftarrow}}

\global\long\def\argPar#1#2{\argrel{#1}{#2}{\Rightarrow}}

\global\long\def\argParinv#1#2{\argrel{#1}{#2}{\Leftarrow}}

\global\long\def\argreds#1#2{\argrel{#1}{#2}{\vartriangleright^{\ast}}}

\global\long\def\argredinvs#1#2{\argrel{#1}{#2}{\vartriangleleft^{\ast}}}

\global\long\def\argReds#1#2{\argrel{#1}{#2}{\rightarrow^{\ast}}}

\global\long\def\argRedinvs#1#2{\argrel{#1}{#2}{\leftarrow^{\ast}}}

\global\long\def\argPars#1#2{\argrel{#1}{#2}{\Rightarrow^{\ast}}}

\global\long\def\argParinvs#1#2{\argrel{#1}{#2}{\Leftarrow^{\ast}}}

\global\long\def\argeq#1#2{\argrel{#1}{#2}{\simeq}}

\global\long\def\argneq#1#2{\iffontspec\argrel{#1}{#2}{\nsimeq}\else\argrel{#1}{#2}{\not\simeq}\fi}

\global\long\def\machred#1{\succ_{#1}}

\global\long\def\machredinv#1{\prec_{#1}}


